Quantum Phase Transition of Non-Hermitian Systems using Variational Quantum Techniques

The motivation for studying non-Hermitian systems and the role of $\mathcal{PT}$-symmetry is discussed. We investigate the use of a quantum algorithm to find the eigenvalues and eigenvectors of non-Hermitian Hamiltonians, with applications to quantum phase transitions. We use a recently proposed variational algorithm. The systems studied are the transverse Ising model with both a purely real and a purely complex transverse field.

==> draftAccuracy.tex <==
\subsection{Hermitian Ising Model}\label{sec:TIM}
To show that our method is suitable for studying the phase transitions of these non-Hermitian systems, we will first test it on the simple transverse Ising chain. The Hamiltonian defining this model is
\begin{equation}\label{eq:TIM}
    \hat{H} = -\sum_{j=0}^{n-1}\left[\sigma_z^j\sigma_z^{j+1} + \Gamma\sigma_x^j\right],
\end{equation}
making use of periodic boundary conditions. This system is well known to have a phase transition in $\Gamma$ \cite{Sachdev2011}. This can be shown by studying the magnetization in the transverse direction. This can be done by finding the groundstate ($|\phi_0\rangle$) and measuring the value of
\begin{equation}\label{eq:Mx}
    \langle \phi_0|\hat{M}_x|\phi_0\rangle = \frac{1}{n}\sum_{j=0}^{n-1}\langle\phi_0|\sigma_x^j|\phi_0\rangle.
\end{equation}
We can produce the plot of this as shown in Fig. \ref{fig:CTIM_Comparison} using the method from Sec. \ref{sec:VQA}. Due to quantum resource limitations, we test this on five spin sites. In the infinite volume limit, we would expect the phase transition to occur at $\Gamma=1$.
